GENCNIPPET: Automated Generation of Code Snippets for Supporting Programming Questions

Context: Software developers often ask questions on Technical Q&A forums like Stack Overflow (SO) to seek solutions to their programming-related problems (e.g., errors and unexpected behavior of code). Problem: Many questions miss required code snippets due to the lack of readily available code, time constraints, employer restrictions, confidentiality concerns, or uncertainty about what code to share. Unfortunately, missing but required code snippets prevent questions from getting prompt and appropriate solutions. Objective: We plan to introduce GENCNIPPET, a tool designed to integrate with SO's question submission system. GENCNIPPET will generate relevant code examples (when required) to support questions for their timely solutions. Methodology: We first downloaded the SO April 2024 data dump, which contains 1.94 million questions related to Python that have code snippets and 1.43 million questions related to Java. Then, we filter these questions to identify those that genuinely require code snippets using a state-of-the-art machine learning model. Next, we select questions with positive scores to ensure high-quality data. Our plan is to fine-tune Llama-3 models (e.g., Llama-3-8B), using 80% of the selected questions for training and 10% for validation. The primary reasons for choosing Llama models are their open-source accessibility and robust fine-tuning capabilities, which are essential for deploying a freely accessible tool. GENCNIPPET will be integrated with the SO question submission system as a browser plugin. It will communicate with the fine-tuned model to generate code snippets tailored to the target questions. The effectiveness of the generated code examples will be assessed using automatic evaluation against ground truth, user perspectives, and live (wild) testing in real-world scenarios.

==> boxplot-acc-ans-score.tex <==

\begin{figure}[!htp]
\centering
        \resizebox{3in}{!}{%
        \begin{tikzpicture}
        \begin{axis}[xmin=0,width=3in,height=3in,
          ylabel = {Score},
          xtick = {1, 2, 3},
          xticklabels = {MICO, COAC, CODS},
          %every axis plot/.append style = {fill, fill opacity = .1}
          ]
        % somewhen the simple statement of `hide outliers` broke.
        % Now the full path to the style needs to be written.
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.0,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        -1\\
        -2\\
        -1\\
        1\\
        1\\
        0\\
        -3\\
        -1\\
        2\\
        -2\\
        2\\
        1\\
        0\\
        -1\\
        1\\
        0\\
        2\\
        3\\
        1\\
        2\\
        1\\
        -1\\
        0\\
        3\\
        1\\
        0\\
        1\\
        0\\
        -2\\
        0\\
        2\\
        -2\\
        0\\
        1\\
        4\\
        -2\\
        0\\
        0\\
        0\\
        3\\
        0\\
        -1\\
        2\\
        7\\
        0\\
        1\\
        -4\\
        1\\
        0\\
        0\\
        0\\
        2\\
        1\\
        1\\
        0\\
        0\\
        0\\
        -1\\
        -1\\
        -1\\
        -7\\
        -2\\
        0\\
        0\\
        3\\
        0\\
        0\\
        -1\\
        5\\
        2\\
        -3\\
        -1\\
        -2\\
        -1\\
        1\\
        -5\\
        0\\
        0\\
        -1\\
        0\\
        0\\
        0\\
        1\\
        -3\\
        -1\\
        1\\
        0\\
        1\\
        1\\
        0\\
        0\\
        -6\\
        6\\
        1\\
        0\\
        };
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.1,
                  black]
        table[row sep=\\,y index=0] {
        data\\
            0\\
            10\\
            8\\
            0\\
            1\\
            0\\
            1\\
            12\\
            0\\
            0\\
            1\\
            1\\
            7\\
            3\\
            -1\\
            0\\
            1\\
            1\\
            0\\
            0\\
            9\\
            0\\
            1\\
            0\\
            5\\
            1\\
            -2\\
            1\\
            0\\
            1\\
            3\\
            0\\
            1\\
            -5\\
            0\\
            1\\
            -3\\
            2\\
            2\\
            4\\
            0\\
            -1\\
            1\\
            8\\
            -2\\
            -1\\
            0\\
            2\\
            0\\
            0\\
            1\\
            2\\
            0\\
            0\\
            2\\
            2\\
            4\\
            1\\
            -1\\
            2\\
            -2\\
            1\\
            0\\
            1\\
            0\\
            0\\
            1\\
            2\\
            1\\
            1\\
            4\\
            0\\
            0\\
            0\\
            5\\
            0\\
            0\\
            2\\
            0\\
            -1\\
            1\\
            1\\
            0\\
            2\\
            0\\
            0\\
            2\\
            0\\
            1\\
            -2\\
            2\\
            -1\\
            -2\\
            0\\
            1\\
            22\\
            0\\
            2\\
            0\\
            0\\
            1\\
            -1\\
            -1\\
            -5\\
            1\\
            0\\
            -1\\
            0\\
            1\\
            -1\\
            0\\
            1\\
            4\\
            0\\
            0\\
            0\\
            0\\
            1\\
            0\\
            0\\
            0\\
            1\\
            9\\
            0\\
            -1\\
            1\\
            1\\
            0\\
            0\\
            0\\
            -2\\
            0\\
            0\\
            4\\
            -1\\
            -1\\
            -1\\
            -1\\
            1\\
            0\\
            -3\\
            0\\
            0\\
            0\\
            1\\
            2\\
            1\\
            0\\
            1\\
            0\\
            2\\
            0\\
            0\\
            0\\
            9\\
            1\\
            -1\\
            0\\
            1\\
            3\\
            1\\
            0\\
            0\\
            0\\
            2\\
            -2\\
            1\\
            0\\
            0\\
            0\\
            };
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.2,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        13\\
        1\\
        35\\
        73\\
        8\\
        3\\
        14\\
        13\\
        4\\
        2\\
        4\\
        7\\
        169\\
        10\\
        13\\
        12\\
        5\\
        7\\
        2\\
        582\\
        1\\
        803\\
        187\\
        97\\
        334\\
        10\\
        5\\
        0\\
        71\\
        24\\
        13\\
        21\\
        20\\
        14\\
        47\\
        346\\
        11\\
        4\\
        49\\
        13\\
        32\\
        41\\
        6\\
        1\\
        16\\
        15\\
        18\\
        4\\
        6\\
        1\\
        6\\
        -3\\
        0\\
        12\\
        1\\
        4\\
        6\\
        0\\
        1\\
        0\\
        2\\
        3\\
        3\\
        4\\
        1\\
        0\\
        6\\
        1\\
        0\\
        0\\
        1\\
        2\\
        0\\
        0\\
        0\\
        0\\
        33\\
        3\\
        0\\
        0\\
        2\\
        4\\
        0\\
        7\\
        5\\
        3\\
        8\\
        6\\
        1\\
        11\\
        0\\
        0\\
        8\\
        1\\
        5\\
        3\\
        1\\
        1\\
        0\\
        1\\
        2\\
        1\\
        0\\
        0\\
        1\\
        0\\
        0\\
        3\\
        0\\
        2\\
        6\\
        0\\
        15\\
        0\\
        0\\
        0\\
        25\\
        0\\
        4\\
        19\\
        1\\
        10\\
        0\\
        0\\
        0\\
        1\\
        1\\
        2\\
        2\\
        8\\
        1\\
        5\\
        0\\
        1\\
        2\\
        1\\
        4\\
        2\\
        11\\
        1\\
        2\\
        0\\
        0\\
        68\\
        3\\
        0\\
        0\\
        1\\
        1\\
        13\\
        2\\
        1\\
        16\\
        0\\
        6\\
        0\\
        3\\
        1\\
        0\\
        0\\
        1\\
        0\\
        0\\
        0\\
        0\\
        2\\
        0\\
        0\\
        9\\
        -2\\
        0\\
        0\\
        1\\
        0\\
        3\\
        0\\
        6\\
        1\\
        19\\
        0\\
        -1\\
        0\\
        3\\
        0\\
        3\\
        0\\
        0\\
        1005\\
        1\\
        4\\
        12\\
        0\\
        4\\
        6\\
        2\\
        -5\\
        0\\
        4\\
        0\\
        5\\
        4\\
        63\\
        2\\
        0\\
        1\\
        -2\\
        2\\
        0\\
        2\\
        3\\
        0\\
        0\\
        1\\
        0\\
        3\\
        0\\
        1\\
        7\\
        1\\
        1\\
        1\\
        1\\
        3\\
        0\\
        0\\
        1\\
        5\\
        1\\
        1\\
        0\\
        0\\
        -1\\
        0\\
        -1\\
        1\\
        2\\
        -1\\
        -1\\
        0\\
        1\\
        1\\
        0\\
        2\\
        -2\\
        0\\
        3\\
        0\\
        0\\
        0\\
        1\\
        };
        \end{axis}
        \end{tikzpicture}
        }
% \vspace{-2mm}
\caption{Score of accepted answer (\texttt{MICO} = Missing Code; \texttt{COAC} = Code After Comment; \texttt{CODS} = Code During  Submission)}
% \vspace{-3mm}
\label{fig:score-acc-ans}
\end{figure}

==> boxplot-delay-adding-code.tex <==

\begin{figure}[!htp]
\centering
        \resizebox{3in}{!}{%

        \begin{tikzpicture}
        \begin{axis}[xmin=0,width=3in,height=3in,
          ylabel = {Time delay (in minutes)},
          xtick = {1, 2, 3},
          xticklabels = {No Answer, Unresolved, Resolved},
          %every axis plot/.append style = {fill, fill opacity = .1}
          ]
        % somewhen the simple statement of `hide outliers` broke.
        % Now the full path to the style needs to be written.
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.0,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        34\\
        5\\
        6\\
        609\\
        8\\
        38\\
        21\\
        799\\
        38\\
        2\\
        728\\
        16\\
        10\\
        32\\
        4\\
        799\\
        13\\
        1\\
        975\\
        7\\
        1403\\
        15\\
        84\\
        2023\\
        15\\
        16\\
        20\\
        1172\\
        1249\\
        2370\\
        865\\
        1\\
        2\\
        4351\\
        15\\
        13\\
        9\\
        456\\
        4\\
        6\\
        1412\\
        100\\
        10\\
        398\\
        2975\\
        35\\
        15\\
        17\\
        134\\
        17\\
        991\\
        23\\
        16\\
        1086\\
        7\\
        310\\
        2\\
        2512\\
        52\\
        835\\
        12\\
        49\\
        20\\
        7\\
        9006\\
        1879\\
        12\\
        3\\
        913\\
        1847\\
        5\\
        10\\
        885\\
        942\\
        11\\
        7\\
        9\\
        24\\
        10\\
        144\\
        };
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.1,
                  black]
        table[row sep=\\,y index=0] {
        data\\
            0\\
            0\\
            0\\
            0\\
            0\\
            1\\
            1\\
            1\\
            1\\
            1\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            6\\
            6\\
            6\\
            6\\
            6\\
            6\\
            6\\
            6\\
            6\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            9\\
            9\\
            9\\
            9\\
            9\\
            9\\
            9\\
            9\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            11\\
            11\\
            11\\
            11\\
            11\\
            11\\
            11\\
            11\\
            11\\
            12\\
            12\\
            12\\
            12\\
            12\\
            12\\
            12\\
            12\\
            13\\
            13\\
            13\\
            13\\
            13\\
            13\\
            13\\
            13\\
            14\\
            14\\
            14\\
            15\\
            15\\
            15\\
            15\\
            15\\
            15\\
            15\\
            16\\
            16\\
            16\\
            17\\
            17\\
            17\\
            17\\
            18\\
            18\\
            20\\
            20\\
            20\\
            20\\
            20\\
            21\\
            21\\
            22\\
            22\\
            22\\
            22\\
            22\\
            22\\
            22\\
            23\\
            23\\
            23\\
            23\\
            23\\
            23\\
            25\\
            25\\
            25\\
            26\\
            26\\
            26\\
            26\\
            27\\
            28\\
            28\\
            28\\
            29\\
            29\\
            29\\
            30\\
            30\\
            31\\
            31\\
            32\\
            32\\
            32\\
            32\\
            32\\
            33\\
            33\\
            35\\
            36\\
            36\\
            36\\
            39\\
            39\\
            40\\
            40\\
            41\\
            43\\
            43\\
            44\\
            44\\
            45\\
            46\\
            49\\
            49\\
            50\\
            50\\
            51\\
            51\\
            51\\
            54\\
            55\\
            59\\
            60\\
            60\\
            61\\
            63\\
            68\\
            69\\
            77\\
            80\\
            83\\
            83\\
            87\\
            93\\
            95\\
            107\\
            109\\
            115\\
            136\\
            146\\
            147\\
            155\\
            157\\
            160\\
            160\\
            162\\
            169\\
            172\\
            184\\
            206\\
            209\\
            215\\
            216\\
            219\\
            229\\
            231\\
            232\\
            243\\
            355\\
            376\\
            447\\
            456\\
            496\\
            502\\
            701\\
            745\\
            843\\
            959\\
            994\\
            999\\
            1069\\
            1070\\
            1076\\
            1158\\
            1274\\
            1321\\
            1450\\
            1585\\
            1609\\
            1680\\
            1688\\
            1918\\
            2540\\
            2721\\
            3843\\
            5060\\
            5317\\
            5714\\
            8244\\
            18786\\
            };
            
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.2,
                  black]
        table[row sep=\\,y index=0] {
        data\\
            2\\
            355\\
            447\\
            21\\
            10\\
            7\\
            2\\
            29\\
            95\\
            5\\
            25\\
            1609\\
            4\\
            4\\
            61\\
            8\\
            6\\
            44\\
            50\\
            8\\
            206\\
            12\\
            11\\
            9\\
            35\\
            7\\
            10\\
            9\\
            0\\
            7\\
            1\\
            8\\
            6\\
            2\\
            7\\
            209\\
            115\\
            4\\
            14\\
            157\\
            5\\
            10\\
            160\\
            36\\
            51\\
            8\\
            11\\
            20\\
            6\\
            0\\
            1\\
            14\\
            83\\
            15\\
            1076\\
            17\\
            376\\
            15\\
            0\\
            5\\
            16\\
            6\\
            17\\
            68\\
            60\\
            26\\
            16\\
            28\\
            12\\
            4\\
            22\\
            26\\
            3\\
            30\\
            12\\
            5\\
            12\\
            155\\
            11\\
            1918\\
            229\\
            5\\
            22\\
            5\\
            7\\
            11\\
            6\\
            10\\
            31\\
            29\\
            843\\
            10\\
            5714\\
            8\\
            1585\\
            2\\
            22\\
            26\\
            15\\
            5060\\
            41\\
            49\\
            8\\
            2\\
            27\\
            4\\
            1\\
            2\\
            9\\
            3\\
            20\\
            2\\
            3\\
            3\\
            10\\
            80\\
            22\\
            502\\
            959\\
            33\\
            701\\
            11\\
            4\\
            172\\
            232\\
            43\\
            2\\
            18\\
            8\\
            1069\\
            5\\
            4\\
            1\\
            5\\
            7\\
            2\\
            20\\
            3\\
            51\\
            60\\
            21\\
            23\\
            8\\
            6\\
            0\\
            4\\
            15\\
            7\\
            2721\\
            3\\
            4\\
            14\\
            8\\
            39\\
            13\\
            20\\
            4\\
            3\\
            11\\
            10\\
            87\\
            3\\
            31\\
            51\\
            25\\
            6\\
            10\\
            40\\
            18\\
            5\\};
        \end{axis}
        \end{tikzpicture}
        }
% \vspace{-2mm}
\caption{Time delay between comment \& code addition by editing.}
% \vspace{-3mm}
\label{fig:time-delay-adding-code}
\end{figure}

==> boxplot-number-of-answers.tex <==

\begin{figure}[!htp]
\centering
        \resizebox{3in}{!}{%

        \begin{tikzpicture}
        \begin{axis}[xmin=0,width=3in,height=3in,
          ylabel = {\# of answers},
          xtick = {1, 2, 3},
          xticklabels = {MICO, COAC, CODS},
          %every axis plot/.append style = {fill, fill opacity = .1}
          ]
        % somewhen the simple statement of `hide outliers` broke.
        % Now the full path to the style needs to be written.
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.0,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        4\\
        4\\
        4\\
        4\\};
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.1,
                  black]
        table[row sep=\\,y index=0] {
        data\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            5\\
            5\\
            5\\
            6\\
            8\\
            };
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.2,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        3\\
        10\\
        10\\
        2\\
        16\\
        7\\
        16\\
        10\\
        5\\
        5\\
        2\\
        1\\
        6\\
        6\\
        5\\
        6\\
        14\\
        14\\
        4\\
        13\\
        8\\
        2\\
        1\\
        5\\
        3\\
        26\\
        2\\
        50\\
        13\\
        10\\
        16\\
        2\\
        2\\
        1\\
        3\\
        7\\
        6\\
        5\\
        2\\
        7\\
        2\\
        2\\
        4\\
        10\\
        2\\
        1\\
        1\\
        9\\
        0\\
        1\\
        1\\
        3\\
        3\\
        4\\
        4\\
        3\\
        4\\
        1\\
        3\\
        1\\
        3\\
        3\\
        0\\
        4\\
        2\\
        2\\
        1\\
        1\\
        2\\
        1\\
        0\\
        1\\
        4\\
        4\\
        2\\
        2\\
        3\\
        3\\
        3\\
        1\\
        1\\
        1\\
        0\\
        1\\
        1\\
        2\\
        1\\
        1\\
        4\\
        0\\
        1\\
        0\\
        1\\
        0\\
        1\\
        1\\
        2\\
        2\\
        1\\
        0\\
        2\\
        1\\
        1\\
        1\\
        2\\
        1\\
        3\\
        2\\
        0\\
        1\\
        2\\
        5\\
        1\\
        2\\
        1\\
        1\\
        0\\
        1\\
        0\\
        2\\
        1\\
        1\\
        1\\
        1\\
        4\\
        1\\
        3\\
        0\\
        0\\
        2\\
        2\\
        0\\
        1\\
        0\\
        1\\
        7\\
        2\\
        4\\
        3\\
        3\\
        0\\
        1\\
        0\\
        1\\
        0\\
        1\\
        1\\
        2\\
        1\\
        1\\
        3\\
        0\\
        3\\
        0\\
        4\\
        0\\
        2\\
        1\\
        1\\
        2\\
        1\\
        1\\
        3\\
        3\\
        2\\
        2\\
        1\\
        1\\
        3\\
        1\\
        3\\
        1\\
        1\\
        1\\
        4\\
        1\\
        1\\
        2\\
        1\\
        2\\
        2\\
        3\\
        2\\
        1\\
        1\\
        1\\
        2\\
        1\\
        1\\
        1\\
        0\\
        2\\
        2\\
        1\\
        2\\
        2\\
        1\\
        2\\
        1\\
        1\\
        7\\
        0\\
        1\\
        1\\
        1\\
        1\\
        4\\
        2\\
        2\\
        1\\
        1\\
        2\\
        1\\
        1\\
        1\\
        5\\
        3\\
        1\\
        0\\
        3\\
        4\\
        1\\
        2\\
        1\\
        1\\
        1\\
        1\\
        3\\
        1\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        3\\
        5\\
        1\\
        1\\
        3\\
        2\\
        1\\
        2\\
        1\\
        12\\
        3\\
        2\\
        1\\
        1\\
        4\\
        1\\
        1\\
        1\\
        5\\
        1\\
        2\\
        1\\
        2\\
        1\\
        0\\
        1\\
        2\\
        1\\
        1\\
        3\\
        0\\
        2\\
        2\\
        1\\
        2\\
        5\\
        2\\
        1\\
        2\\
        1\\
        4\\
        0\\
        2\\
        1\\
        1\\
        1\\
        1\\
        7\\
        1\\
        1\\
        1\\
        2\\
        1\\
        0\\
        1\\
        2\\
        3\\
        2\\
        2\\
        1\\
        1\\
        4\\
        1\\
        2\\
        3\\
        3\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        1\\
        9\\
        1\\
        3\\
        4\\
        2\\
        1\\
        1\\
        7\\
        1\\
        2\\
        1\\
        1\\
        1\\
        2\\
        1\\
        2\\
        6\\
        2\\
        4\\
        1\\
        1\\
        2\\
        1\\
        2\\
        0\\
        1\\
        0\\
        1\\
        0\\
        1\\
        1\\
        1\\
        2\\
        1\\
        1\\
        1\\
        3\\
        1\\
        1\\
        0\\
        2\\
        1\\
        0\\
        1\\
        3\\
        1\\
        4\\
        2\\
        0\\
        2\\
        1\\
        1\\
        2\\
        1\\
        3\\
        2\\
        2\\
        1\\
        0\\
        1\\
        2\\
        0\\
        1\\
        1\\
        1\\
        1\\
        3\\
        1\\
        2\\
        2\\
        3\\
        1\\
        3\\
        2\\
        1\\
        3\\
        2\\
        2\\
        1\\
        1\\
        1\\
        1\\
        3\\
        3\\
        1\\
        1\\
        2\\
        4\\
        3\\
        1\\
        1\\
        1\\
        1\\
        2\\
        1\\
        2\\
        2\\
        2\\
        };
        
        \end{axis}
        \end{tikzpicture}
        }
% \vspace{-2mm}
\caption{Number of answers (\texttt{MICO} = Missing Code; \texttt{COAC} = Code After Comment; \texttt{CODS} = Code During  Submission)}
% \vspace{-3mm}
\label{fig:no-of-answers}
\end{figure}

==> boxplot-time-delay-receiving-acc-ans.tex <==

\begin{figure}[!htp]
\centering
        \resizebox{3.3in}{!}{%

        \begin{tikzpicture}
        \begin{axis}[xmin=0,width=3.5in,height=3.5in,
          ylabel = {Time delay (in minutes)},
          xtick = {1, 2, 3, 4},
          xticklabels = {MICO, COAC, COAC*, CODS},
          %every axis plot/.append style = {fill, fill opacity = .1}
          ]
        % somewhen the simple statement of `hide outliers` broke.
        % Now the full path to the style needs to be written.
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.0,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        83\\
        496\\
        7\\
        542\\
        169\\
        849\\
        29\\
        30\\
        47\\
        41\\
        20\\
        29\\
        3\\
        2\\
        96\\
        568\\
        3358\\
        1072\\
        45\\
        217144\\
        4535\\
        9\\
        106\\
        123941\\
        80\\
        3\\
        214\\
        1235\\
        10\\
        418\\
        217\\
        42\\
        51\\
        143\\
        11459\\
        104\\
        446\\
        41\\
        191\\
        155\\
        10416\\
        40\\
        1645\\
        42\\
        6\\
        2369\\
        10\\
        61\\
        1065\\
        22\\
        159\\
        17\\
        663\\
        29\\
        711\\
        1650\\
        74\\
        30\\
        1\\
        24\\
        10\\
        9825\\
        41\\
        71\\
        191\\
        48\\
        62\\
        5\\
        232\\
        4\\
        5\\
        17\\
        28\\
        14\\
        35\\
        23\\
        35\\
        106200\\
        433\\
        7\\
        576472\\
        185\\
        4\\
        26\\
        4\\
        386\\
        4155\\
        38\\
        39\\
        5\\
        461\\
        15\\
        13\\
        28\\
        73\\
        };
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.1,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        248\\
        79\\
        125\\
        5209\\
        42\\
        80\\
        529\\
        6028\\
        1140\\
        30\\
        54\\
        170\\
        3185\\
        317\\
        13\\
        68\\
        33\\
        5\\
        19\\
        1997338\\
        71\\
        22\\
        57\\
        1468\\
        766\\
        17\\
        25\\
        995\\
        29\\
        3436\\
        248\\
        72\\
        28\\
        22\\
        3691\\
        2758\\
        28\\
        56\\
        40\\
        30\\
        14\\
        31\\
        47\\
        3522\\
        159\\
        47\\
        14\\
        105\\
        4827\\
        17\\
        84\\
        81\\
        15\\
        728\\
        44\\
        11\\
        59\\
        16\\
        35\\
        341\\
        28\\
        39\\
        94\\
        97\\
        1319\\
        51\\
        10305\\
        75\\
        2336\\
        92\\
        747\\
        22\\
        3274\\
        10\\
        335\\
        238\\
        22\\
        185\\
        601\\
        75\\
        126\\
        227\\
        220\\
        878\\
        142\\
        10\\
        1033\\
        10\\
        305\\
        45\\
        183\\
        4752\\
        16\\
        86\\
        38\\
        730\\
        15\\
        1022\\
        18\\
        372\\
        37\\
        4660\\
        3116\\
        1090\\
        71\\
        720\\
        30\\
        43\\
        186\\
        1551\\
        48\\
        1184\\
        180\\
        164\\
        40\\
        3358\\
        27\\
        1023\\
        1794\\
        125\\
        62\\
        24\\
        35\\
        55\\
        32\\
        201\\
        20\\
        43\\
        25\\
        76\\
        126\\
        1835\\
        38\\
        152\\
        26\\
        16\\
        17\\
        117\\
        12\\
        1662\\
        195\\
        37\\
        54\\
        2040\\
        23\\
        107\\
        9\\
        910\\
        87\\
        465\\
        15\\
        101\\
        9\\
        30\\
        24\\
        26\\
        39\\
        18\\
        96\\
        101\\
        50\\
        1475\\
        1427\\
        1130\\
        66\\
        5732\\
        21\\
        3381\\
        35\\
        89\\
        };
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.2,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        232\\
        44\\
        110\\
        2528\\
        19\\
        37\\
        26\\
        464\\
        1102\\
        22\\
        11\\
        126\\
        2456\\
        171\\
        6\\
        18\\
        30\\
        2\\
        16\\
        1997305\\
        17\\
        16\\
        22\\
        1412\\
        649\\
        3\\
        16\\
        987\\
        2\\
        1808\\
        242\\
        67\\
        22\\
        17\\
        3628\\
        31\\
        23\\
        7\\
        25\\
        22\\
        8\\
        23\\
        1\\
        3508\\
        107\\
        27\\
        8\\
        73\\
        4238\\
        13\\
        52\\
        31\\
        5\\
        691\\
        21\\
        6\\
        20\\
        0\\
        15\\
        37\\
        18\\
        5\\
        13\\
        92\\
        1229\\
        33\\
        3703\\
        71\\
        1372\\
        54\\
        21\\
        11\\
        3259\\
        1\\
        291\\
        15\\
        8\\
        61\\
        595\\
        60\\
        86\\
        212\\
        10\\
        830\\
        92\\
        3\\
        868\\
        6\\
        5\\
        6\\
        118\\
        4743\\
        4\\
        61\\
        18\\
        520\\
        13\\
        331\\
        5\\
        8\\
        20\\
        95\\
        3051\\
        13\\
        4\\
        331\\
        12\\
        7\\
        146\\
        1493\\
        41\\
        112\\
        157\\
        121\\
        3\\
        1527\\
        23\\
        958\\
        691\\
        89\\
        27\\
        12\\
        26\\
        20\\
        15\\
        195\\
        4\\
        19\\
        7\\
        26\\
        38\\
        1795\\
        31\\
        73\\
        18\\
        1\\
        10\\
        50\\
        5\\
        1580\\
        34\\
        20\\
        28\\
        102\\
        2\\
        81\\
        4\\
        850\\
        21\\
        187\\
        1\\
        77\\
        2\\
        11\\
        11\\
        3\\
        0\\
        4\\
        75\\
        66\\
        19\\
        1444\\
        1342\\
        277\\
        39\\
        12\\
        7\\
        1786\\
        25\\
        48\\
        };
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.3,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        9\\
        250\\
        2\\
        7\\
        18\\
        5\\
        326686\\
        71\\
        1584\\
        2\\
        12\\
        20\\
        2\\
        60\\
        59\\
        49\\
        5\\
        65\\
        12\\
        1075885\\
        3\\
        5\\
        1035492\\
        16\\
        288534\\
        264\\
        5\\
        663\\
        10\\
        11\\
        85\\
        559\\
        10\\
        17\\
        26\\
        9\\
        42\\
        550\\
        5\\
        380\\
        7\\
        7\\
        27\\
        12\\
        11\\
        8\\
        118\\
        95\\
        559\\
        317\\
        41\\
        3\\
        5\\
        445\\
        963\\
        3074\\
        1422\\
        182\\
        3475\\
        4009\\
        449\\
        21\\
        3367\\
        323\\
        390\\
        3926\\
        1876\\
        2111\\
        3\\
        427\\
        253\\
        2087\\
        19\\
        952\\
        4\\
        1047\\
        4604127\\
        2\\
        853\\
        1469\\
        334\\
        5\\
        20\\
        2\\
        4\\
        216\\
        150\\
        158067\\
        108\\
        51\\
        533\\
        10\\
        147\\
        5\\
        35\\
        13\\
        1\\
        1\\
        11\\
        71\\
        40\\
        691\\
        5\\
        1740\\
        1041\\
        66\\
        202\\
        804351\\
        9\\
        35\\
        5\\
        92\\
        607533\\
        21\\
        647\\
        148\\
        231\\
        19\\
        113\\
        4\\
        17\\
        22\\
        7\\
        892\\
        784\\
        8\\
        282\\
        11\\
        621\\
        7\\
        2\\
        772\\
        12\\
        9\\
        915\\
        21\\
        1040\\
        621\\
        22\\
        18\\
        3\\
        8\\
        151\\
        6\\
        21\\
        10\\
        4\\
        119\\
        6\\
        186\\
        259\\
        283\\
        1299\\
        1333\\
        27\\
        8\\
        956\\
        104\\
        18\\
        41\\
        7\\
        72\\
        198\\
        6\\
        76\\
        4\\
        26\\
        20\\
        4\\
        129\\
        1293\\
        1\\
        21\\
        39\\
        270\\
        13\\
        67\\
        4\\
        675488\\
        6\\
        1\\
        5\\
        4\\
        64\\
        4\\
        109\\
        47\\
        31\\
        5\\
        76\\
        18\\
        12\\
        3\\
        19\\
        4\\
        11\\
        16\\
        16\\
        17\\
        28\\
        243\\
        5\\
        633\\
        4\\
        422\\
        4\\
        5\\
        10\\
        3091\\
        789\\
        2640\\
        2393\\
        1287\\
        126\\
        1841\\
        3108\\
        3\\
        84\\
        538\\
        1907\\
        46\\
        6\\
        35\\
        50\\
        100\\
        11\\
        1287\\
        38\\
        6\\
        44\\
        39\\
        5\\
        18\\
        1\\
        28\\
        1\\
        4\\
        19\\
        3\\
        4\\
        9\\
        10\\
        6\\
        4\\
        8\\
        62\\
        5\\
        10\\
        2\\
        7\\
        };
        \end{axis}
        \end{tikzpicture}
        }
% \vspace{-2mm}
\caption{Time delay of receiving accepted answer (\texttt{MICO} = Missing Code; \texttt{COAC} = Code After Comment; \texttt{COAC\textsuperscript{*}} = COAC regarding the editing time to add code; \texttt{CODS} = Code During  Submission)}
% \vspace{-3mm}
\label{fig:delay-receiving-acc-ans}
\end{figure}
